Bora: Biomedical Generalist Video Generation Model

Generative models hold promise for revolutionizing medical education, robot-assisted surgery, and data augmentation for medical AI development. Diffusion models can now generate realistic images from text prompts, while recent advancements have demonstrated their ability to create diverse, high-quality videos. However, these models often struggle with generating accurate representations of medical procedures and detailed anatomical structures. This paper introduces Bora, the first spatio-temporal diffusion probabilistic model designed for text-guided biomedical video generation. Bora leverages Transformer architecture and is pre-trained on general-purpose video generation tasks. It is fine-tuned through model alignment and instruction tuning using a newly established medical video corpus, which includes paired text-video data from various biomedical fields. To the best of our knowledge, this is the first attempt to establish such a comprehensive annotated biomedical video dataset. Bora is capable of generating high-quality video data across four distinct biomedical domains, adhering to medical expert standards and demonstrating consistency and diversity. This generalist video generative model holds significant potential for enhancing medical consultation and decision-making, particularly in resource-limited settings. Additionally, Bora could pave the way for immersive medical training and procedure planning. Extensive experiments on distinct medical modalities such as endoscopy, ultrasound, MRI, and cell tracking validate the effectiveness of our model in understanding biomedical instructions and its superior performance across subjects compared to state-of-the-art generation models.

==> weixiang/con.tex <==
\section{Conclusion}

We introduce Bora, a model specifically designed for generating biomedical videos. To build this model, we leveraged GPT-4's powerful performance in the biomedical and video domain along with detailed descriptions and background knowledge from video data, creating the first high-quality biomedical text-video pair dataset. Bora demonstrates state-of-the-art accuracy and authenticity in generating biomedical videos, while also achieving excellent overall video quality.

However, despite Bora representing a significant step forward in biomedical video generation, it remains highly constrained by the quality of data and captions. Although GPT-4 is proficient in the biomedical field, it is still insufficient to fully support "accurate, professional" captions. In the future, we will continue to optimize dataset quality and iterate more advanced model architectures.

==> weixiang/res.tex <==
\subsection{Results}


The evaluation results of biomedical instruction following ability are shown in Table~\ref{tab: following ability}. It can be observed that our Bora significantly outperforms other models across all metrics. It should be noted that BERT~\cite{bert} maps text into an embedding space and performs comparisons based on vectors, it does not operate based on actual semantics. The BmU (Biomedical understanding) of other models is already at a considerably low level, resulting in the generated videos being almost entirely different. The comparison of video between Bora and other models is shown in Figure~\ref{fig: compare}.

Due to the significant discrepancies in the evaluation results from the previous phase, it is deemed unnecessary to conduct further comprehensive quality assessments on videos generated by other models. On one hand, comparing models that do not specialize in the biomedical domain is not fair; on the other hand, the biomedical videos they produce do not accurately reflect their true performance. Therefore, we shift our focus to evaluating videos generated across the four modalities we cover. For a concise and intuitive comparison of data, we still incorporate the evaluation results of Sora~\cite{yuan2024mora}. The results of comprehensive video quality are illustrated in Table~\ref{tab: quality}

In terms of Subject Consistency, cell leads by a significant margin. This actually reflects that we have not addressed the issue of minimal inter-frame variation in the cell domain, resulting in videos where the subject remains largely unchanged. The same applies to the Dynamic Degree. Moreover, other metrics show little variation across the four modalities and generally perform well. The Image Quality of the Endoscope even slightly surpasses that of Sora. Despite some performance discrepancies between different modalities, the average scores still demonstrate its performance approaching that of Sora.

==> weixiang/rw.tex <==
\textbf{Medical Generation. }
In recent years, the application of generative models has expanded significantly, evolving from conventional domains to specialized industries, including the field of biomedicine. Specifically, Generative Adversarial Networks (GANs) have been employed to produce high-quality medical images such as MR~\cite{han2018gan}, CT~\cite{emami2021sa,liang2019generating}, and X-ray images~\cite{madani2018chest,motamed2021data}. For some rare diseases, these generated images effectively augment data availability, enhancing both physicians' and algorithms' ability to recognize and understand the characteristics of these conditions~\cite{lee2022deep,sanchez2020deep,madani2018chest}. In terms of privacy protection, while adhering to stringent data privacy regulations such as GDPR~\cite{gdpr} or HIPAA~\cite{HIPAA,baumer2000privacy}, generative models can create anonymized medical data. These datasets maintain statistical similarities to real data but do not contain personally identifiable information, thus allowing researchers to conduct studies and analyses without violating patient privacy~\cite{baowaly2019synthesizing,yoon2020anonymization}. Generative models transcend the confines of traditional applications and are highly integrated with specific subfields in biomedicine. In drug development, generative models can predict molecular activity, aiding scientists in designing new pharmaceutical molecules, thereby significantly accelerating the early stages of drug discovery and optimization~\cite{mak2023artificial,gentile2022artificial,guan2022class,jiang2022sequence,kim2019drug}. Additionally, these models can predict protein structures and interactions, which are crucial for understanding disease mechanisms and developing targeted therapeutic strategies~\cite{varadi2022alphafold,jumper2021highly,lin2023evolutionary,yang2023alphafold2}. However, in the realm of video, only Endora~\cite{endora} has made preliminary explorations in the field of generating medical videos from images. To further advance the development of biomedical videos, we propose a generative model, Bora, akin to Sora, capable of producing high-quality and accurate biomedical videos, thus laying the groundwork for unlocking the potential of biomedical generative video.

==> xiaocao/intro.tex <==
 \section{Introduction}
Generative AI technologies have stepped into a new era, fundamentally altering how industries operate and deeply influencing everyday life~\cite{GPT4report}. Text-to-image (T2I) diffusion models are now capable of generating realistic images that adhere to complex text prompts~\cite{saharia2022photorealistic, rombach2022high}. Recent video generation models like Pika~\cite{pika}, SVD~\cite{SVD} and Gen-2~\cite{Gen-2} have also demonstrated their ability to create diverse and high-quality videos, primarily in general contexts. Sora~\cite{liu2024sora}, introduced by OpenAI in February 2024 and known for its advanced capabilities in generating detailed videos from textual descriptions. It stands out by its capacity to generate high-quality videos lasting up to one minute, while faithfully following the textual instructions provided by the users~\cite{openai2024sora}. Despite their revolutionary capabilities, these models often struggle with generating accurate representations of medical procedures, detailed anatomical structures, and other specific clinical information.

In the biomedical domain, medical image generation has undergone rapid advancement, evolving with diverse models and exhibiting outstanding performance, including retinal image synthesis~\cite{Sindel_2023}, skin lesion synthesis~\cite{Bissoto_2018} and cells image generation~\cite{Liu2021CellsIG}. However, the domain of medical video generation remains notably underdeveloped. Although there are also scarce medical video generation models such as Endora~\cite{endora}, which specializes in creating realistic endoscopy videos, their scope is often limited to a single medical modality. This limitation stems largely from the lack of extensive (text, video) datasets with multiple modalities comparable to those available in general contexts. Additionally, the complexity of certain surgical videos, which contain intricate spatial and temporal details within high-resolution frames, presents further challenges to the development of effective video generation models. Addressing the deficiency is crucial for advancing biomedical applications, as there is a significant need for models capable of generating videos that can support the nuanced requirements of medical diagnostics and research. 

In this paper, we present Bora, the first text-to-video model in the biomedical domain capable of generating videos across four biomedical modalities, exhibiting outstanding quality. Videos generated by Bora have significant potential to enhance clinical practice by providing patients with tailored visual demonstrations and offering medical students invaluable educational resources. Furthermore, Bora serves as a powerful tool for computational biomedical research, helping to bridge gaps due to sample scarcity and facilitating causal inference. Its proficiency in producing realistic biomedical videos also accelerates the integration and development of AR/VR technologies in the biomedical field, opening new avenues for immersive medical training and procedure planning.

% weixiang
Specifically, our paper makes the following contributions:

\begin{itemize}
    \item \textbf{Biomedical Text-Video Pair Dataset: }We propose a novel dataset construction process utilizing open-source biomedical video data. This process leverages GPT-4's capabilities in temporal information and the biomedical domain to create the first biomedical text-video pair dataset, covering four biomedical modalities. Throughout this process, we ensure the retention of video and background information.
    
    \item \textbf{Bora: }In the biomedical domain, we introduce Bora, which efficiently generates accurate, high-quality biomedical videos without the need for training new text encoders or VAEs. Our approach involves a two-stage training process. Initially, we align the modalities covered in the dataset by extracting images from the videos. Subsequently, we train the model using our text-video pair data to enhance its video generation capabilities. Our experiments demonstrate that Bora significantly outperforms other models in terms of accuracy in biomedical video generation, validating the effectiveness of our training process. Additionally, Bora exhibits excellent performance in video quality.
\end{itemize}





==> xiaocao/related_work.tex <==
\section{Related Work}
\textbf{Text-Video Generation.} \quad Recent years have witnessed significant discussion on video generative models. In the initial stages, models predominantly leveraged Variational Autoencoders (VAEs) and Generative Adversarial Networks (GANs)~\cite{li2017video, tulyakov2017mocogan, Chu_2020, yaohui2020imaginator}.Although GANs exhibit advantages in generating realistic videos, their drawbacks of mode collapse and training instability have hampered their progress. In contrast, transformer and diffusion architectures~\cite{vaswani2023attention, ho2020denoising} have demonstrated exceptional performance in the realm of video generation~\cite{blattmann2023stable, chen2023gentron}, capable of generating dynamic and accurate video content from textual prompts.

Originally, diffusion models are designed for image generation~\cite{rombach2022high}, which are adapted to process videos by replacing the image diffusion U-Net with a 3D U-Net structure in the initial trials~\cite{ho2022imagen, singer2022makeavideo}, using  spatial and temporal modules to generate time-consistent videos. Subsequently, MagicVideo~\cite{zhou2023magicvideo} introduces latent diffusion models (LDMs) to the text-to-video generation framework, enhancing model's capabilities to capture dynamics in video contents and generate smooth video clips. The following research by~\cite{ge2023preserve} proposes a video noise prior, leading to enhanced performance in video generation. There are also researchers making efforts to decrease the computational burden during fine-tuning of text-to-video models, such as downsampling the videos spatio-temporally~\cite{bar2024lumiere}.


% \textbf{Medical Generative Data.} \quad Simulated medical data are increasingly being recognized for their valuable applications in medical education, patient care and model training. Synthesized low-resolution images conditioned on text serve as a foundation for subsequent 3D CT images in ~\cite{xu2023medsyn}.
